Imitation Learning for Autonomous Trajectory Learning of Robot Arms in Space

This work adds on to the on-going efforts to provide more autonomy to space robots. Here the concept of programming by demonstration or imitation learning is used for trajectory planning of manipulators mounted on small spacecraft. For greater autonomy in future space missions and minimal human intervention through ground control, a robot arm having 7-Degrees of Freedom (DoF) is envisaged for carrying out multiple tasks like debris removal, on-orbit servicing and assembly. Since actual hardware implementation of microgravity environment is extremely expensive, the demonstration data for trajectory learning is generated using a model predictive controller (MPC) in a physics based simulator. The data is then encoded compactly by Probabilistic Movement Primitives (ProMPs). This offline trajectory learning allows faster reproductions and also avoids any computationally expensive optimizations after deployment in a space environment. It is shown that the probabilistic distribution can be used to generate trajectories to previously unseen situations by conditioning the distribution. The motion of the robot (or manipulator) arm induces reaction forces on the spacecraft hub and hence its attitude changes prompting the Attitude Determination and Control System (ADCS) to take large corrective action that drains energy out of the system. By having a robot arm with redundant DoF helps in finding several possible trajectories from the same start to the same target. This allows the ProMP trajectory generator to sample out the trajectory which is obstacle free as well as having minimal attitudinal disturbances thereby reducing the load on ADCS.

==> src/results.tex <==
\subsection{Experiments in Simulation}
% For our simulation study, a real scene with a table as an obstacle was recorded with Kinect as point-clouds  and was imported to RViz, as shown in \cref{fig:planning_sceneRviz}. The position the robot end-effector has to reach is carefully chosen to be under the table (and the table can be moved in the work space as long as there are enough demonstrations to learn effectively). ProMP, CHOMP and STOMP are implemented in Python whereas RRT is used directly from the Open Motion Planning Library (OMPL) \cite{sucan2012}. The purpose of this is to show that the plan generated by local planners is smoother than sampling-based planners. Quantitatively, the ProMP generated a plan which on average is 52\% and 79\% smoother than CHOMP/STOMP and RRT respectively. The success rate for planning was found to be 87\%, 21\% and 71\% for ProMP, CHOMP and STOMP respectively. This also emphasises that a straight line discretisation of the trajectory has very poor chance of finding a solution. Average planning time to success for local planners was relatively high and is about a minute. This could be attributed to implementation in Python and can be significantly reduced by opting for other programming languages like C/C++. However, from the results obtained, it was clearly demonstrated that for ProMP the average time for successful plan is 17\% and 10\% better than CHOMP and STOMP respectively. All the planners avoid obstacles more or less the same way as seen from the obstacle cost. The small value in \Cref{tab:real_robot_results} is due to the particular value chosen for $\epsilon$ and $k$ in \cref{eq:obs_cost}

% \subsection{Experiments With a Real Robot}
% In addition to the tests in simulation, our algorithm has also been measured using a real 7 DOF Frank Emika's Panda robot. The video attached (or https://www.youtube.com/watch?v=NWx7IXqub5E) shows how the planner goes to a location under the table in two different ways

% \begin{table*}[ht]
% \hspace{1cm}
% \caption{Results of motion planning in simulation}
% \label{tab:real_robot_results}
% \footnotesize
% \centering
% % \settowidth\tymin{\textbf{Scenario}}
% \setlength\extrarowheight{3pt}
% % \begin{tabulary}{0.9\columnwidth}{|c|c|c|c|c|c|}
% \begin{tabulary}{\textwidth}{|c|c|c|c|c|}
% \hline
%     Scenario & 
%     ProMP & Chomp (Straight line input) & 
%     STOMP (stochastic input) & 
%     RRT \\
% \hline
% Number of successful plans & 87/100 & 21/100 & 71/100 & 92/100 \\
% Average planning time to success~(s) & 58.15~$\pm$~11.56 & 68.19~$\pm$~13.42 & 63.99~$\pm$~12.65 & 0.15~$\pm$~0.06 \\
% Average smoothness cost &  0.079~$\pm$~0.0082 & 0.167~$\pm$~0.03 & 0.161~$\pm$~0.03 & 0.377~$\pm$~0.06  \\
% Average obstacle cost & 0.038~$\pm$~0.034 & 0.0165~$\pm$~0.014 & 0.022~$\pm$~0.015 & 0.063~$\pm$~0.022\\\hline
% \end{tabulary}
% \end{table*}
